Conformalizing Machine Translation Evaluation

Several uncertainty estimation methods have been recently proposed for machine translation evaluation. While these methods can provide a useful indication of when not to trust model predictions, we show in this paper that the majority of them tend to underestimate model uncertainty, and as a result they often produce misleading confidence intervals that do not cover the ground truth. We propose as an alternative the use of conformal prediction, a distribution-free method to obtain confidence intervals with a theoretically established guarantee on coverage. First, we demonstrate that split conformal prediction can ``correct'' the confidence intervals of previous methods to yield a desired coverage level. Then, we highlight biases in estimated confidence intervals, both in terms of the translation language pairs and the quality of translations. We apply conditional conformal prediction techniques to obtain calibration subsets for each data subgroup, leading to equalized coverage.

==> intervals.tex <==
\begin{figure*}
\centering
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_original_COMET_MCD.png}
\caption{Original uncertainty}
\label{fig:test1}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_calibration_COMET_MCD.png}
\caption{Calibrated uncertainty}
\label{fig:test2}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_conformal_COMET_MCD.png}
\caption{Conformal prediction}
\label{fig:test3}
\end{minipage}
\end{figure*}


\begin{figure*}
\centering
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_original_COMET_DE.png}
\caption{Original uncertainty}
\label{fig:test1}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_calibration_COMET_DE.png}
\caption{Calibrated uncertainty}
\label{fig:test2}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_conformal_COMET_DE.png}
\caption{Conformal prediction}
\label{fig:test3}
\end{minipage}
\end{figure*}

\begin{figure*}
\centering
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_original_COMET_HTS.png}
\caption{Original uncertainty}
\label{fig:test1}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_calibration_COMET_HTS.png}
\caption{Calibrated uncertainty}
\label{fig:test2}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_conformal_COMET_HTS.png}
\caption{Conformal prediction}
\label{fig:test3}
\end{minipage}
\end{figure*}

\begin{figure*}
\centering
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_original_COMET_DUP.png}
\caption{Original uncertainty}
\label{fig:test1}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_calibration_COMET_DUP.png}
\caption{Calibrated uncertainty}
\label{fig:test2}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\linewidth]{images/confidence_conformal_COMET_DUP.png}
\caption{Conformal prediction}
\label{fig:test3}
\end{minipage}
\end{figure*}

==> mondrian_figure.tex <==
\begin{figure*}
\centering
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_confQUANT.png}
\caption{Coverage over binned DA scores for quantile regression -- conformal prediction}
\label{fig:mondrianqnt_pre}
\end{minipage}\hfill
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_montrian_confQUANT.png}
\caption{Coverage over binned DA scores for quantile regression -- mondrian conformal prediction}
\label{fig:mondrianqnt}
\end{minipage}\\
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_confMCD.png}
\caption{Coverage over binned DA scores for MC dropout -- conformal prediction}
\label{fig:mondrianmcd_pre}
\end{minipage}\hfill
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_montrian_confMCD.png}
\caption{Coverage over binned DA scores for MCD dropout  -- mondrian conformal prediction}
\label{fig:mondrianmcd}
\end{minipage}
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_confDE.png}
\caption{Coverage over binned DA scores for deep ensembles -- conformal prediction}
\label{fig:mondriande_pre}
\end{minipage}\hfill
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_montrian_confDE.png}
\caption{Coverage over binned DA scores for deep ensembles -- mondrian conformal prediction}
\label{fig:mondriande}
\end{minipage}
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_confHTS.png}
\caption{Coverage over binned DA scores for heteroscedastic regression -- conformal prediction}
\label{fig:mondrianhts_pre}
\end{minipage}\hfill
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_montrian_confHTS.png}
\caption{Coverage over binned DA scores for heteroscedastic regression -- mondrian conformal prediction}
\label{fig:mondrianhts}
\end{minipage}

\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_confDUP.png}
\caption{Coverage over binned DA scores for direct uncertainty prediction -- conformal prediction}
\label{fig:mondriandup_pre}
\end{minipage}\hfill
\begin{minipage}{.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/conditional_coverage_zscore_montrian_confDUP.png}
\caption{Coverage over binned DA scores for direct uncertainty prediction -- mondrian conformal prediction}
\label{fig:mondriandup}
\end{minipage}
\end{figure*}


==> stratified.tex <==
Apart from coverage over the full test set we also report the size-stratified coverage (SSC) to ensure that we obtain accurate intervals for the full range of possible interval widths. We hence compute the coverage for binned interval widths; in an ideal scenario, we would want the coverage to be close to $1-\alpha$ for all bins. To compare the deviation for each method, we focus on the minimum coverage obtained per method as  shown in Eq. \ref{eq:ssc}.
%\andre{I'm a bit confused, isn't SSC also a coverage metric? shouldn't we provide some measure of the sharpness to assess how useful our intervals are?}

\begin{equation}
\label{eq:ssc}
    \mathrm{SSC} = \min_{g \in \{1,...,G\}} \frac{1}{\mid I_g\mid} \sum_{i \in I_g} \mathds{1} \{Y_i \in C(X_i)\}
\end{equation}

 for $I_g \subset \{1, \dots , n\}$ being the set of observations falling in bin $g$ for $g = 1, \dots , G$ being bins of different confidence interval sizes. The results can be seen in Table \ref{tab:sha_ssc}. We can observe that for the majority of predictors (except for quantile regression) conformal prediction achieves better SSC values, i.e. more balanced coverage over confidence intervals of different sizes.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c }
         Method & Conformal & Calib. & Orig. $u(\hat{y})$ \\
         QNT & 88.47 & 97.24 & 84.94\\
         MCD & 96.77 & 87.05 & 13.22\\
         DE &  95.82 & 85.04 & 11.04\\
         HTS & 92.96 & 86.52 & 86.26\\
         DUP & 75.95 & 66.08 & 62.63\\
    \end{tabular}
    \caption{Size stratified coverage (averaged over 20 bins per case) for each uncertainty prediction method. }
    \label{tab:sha_ssc}
\end{table}

